Stochastic optimization on matrices and a graphon McKean-Vlasov limit

We consider stochastic gradient descents on the space of large symmetric matrices of suitable functions that are invariant under permuting the rows and columns using the same permutation. We establish deterministic limits of these random curves as the dimensions of the matrices go to infinity while the entries remain bounded. Under a ``small noise'' assumption the limit is shown to be the gradient flow of functions on graphons whose existence was established in Oh, Somani, Pal, and Tripathi, \texit{J Theor Probab 37, 1469--1522 (2024)}. We also consider limits of stochastic gradient descents with added properly scaled reflected Brownian noise. The limiting curve of graphons is characterized by a family of stochastic differential equations with reflections and can be thought of as an extension of the classical McKean-Vlasov limit for interacting diffusions to the graphon setting. The proofs introduce a family of infinite-dimensional exchangeable arrays of reflected diffusions and a novel notion of propagation of chaos for large matrices of diffusions converging to such arrays in a suitable sense.

==> sections/discussion.tex <==
\section{Discussions}
% \subsection{Non-trivial boundary effect}\label{subsec:Discussion}
% It is worth noting that the existence of the boundary $\set{-1,1}$ in our problem makes it non-trivial. To elucidate, consider the following iteration scheme without the boundary projection,
%  \begin{align}\label{eq:NSGD}
%     W_{n,k+1} = W_{n,k} - n^2\tau_{n,k}g_n\round{W_{n,k};\xi_{k+1}} + \tau_{n,k}^{1/2}G_{n,k} ,\qquad k\in\Integer_+ ,\tag{NSGD}
% \end{align}
% starting at some $n\times n$ symmetric matrix $W_{n, 0}$, where $\round{G_{n, k}}_{k\in\Integer_+}$ is a $n\times n$ symmetric matrix valued martingale difference sequence with independent and centered entries. Since for all $k\in\Integer_+$, we have $\lim_{n\to\infty}\cutnorm{G_{n, k}} = 0$, it easily follows that the additive noise does not matter in the limit. But this is not the case when there is a boundary involved as in the iteration scheme~\eqref{eq:PNSGD}. To see this, take the simplest case when $g_n = \nabla \ell_n\equiv 0$, i.e., consider the iteration scheme~\eqref{eq:NSGD} for a constant function $\ell$, say starting at $W_{n, 0}\in\Mcal_n$ (see item~\ref{item:small_noise} in Section~\ref{sec:intro}). The gradient flow in this case should be a constant curve. The corresponding GD iteration would also stay at $W_{n, 0}$ at all times $t\in\R_+$, for each $n\in\Natural$. If we consider the iteration scheme~\eqref{eq:NSGD}, then $W_n$ is a random curve over $n\times n$ symmetric matrices for each $n\in\Natural$ with $\E{W_{n}(t)}=W_{n, 0}$ for all $t\in\R_+$. If $\round{W_{n, 0}}_{n\in\Natural}\to W_0$ in the cut norm $\cutnorm{}$, then $\lim_{n\to \infty}\sup_{t\in\interval{0,T}}\cutnorm{W_n(t)-W_0} = 0$ for any finite $T>0$. But if we consider the iteration scheme~\eqref{eq:PNSGD}, then $\E{W_{n,t}}\neq W_{n, 0}$ except at time $t=0$. Also, it is clear that as $t\to \infty$ and $\abs{\tauvec_n}\to 0$, each element $W_{n}(i, j)(t)$ of $W_n(t)$, since independent for every $(i,j)\in\squarebrack{n}^{2}$, converges to the expectation of the equilibrium distribution of reflecting Brownian motion starting at $W_{n, 0}(i, j)$, as $t\to\infty$. Thus, it becomes clear that $\round{W_n}_{n\in\Natural}$ converges to some curve $W\colon\R_+ \to \Wcal$ appropriately in the limit as $n\to\infty$ that is not a constant curve, in particular, not the gradient flow of $R$.

% Another crucial property that we should note is that as $n\to \infty$, we expect the curves $\round{W_n\colon\R_+\to\Mcal_n}_{n\in\Natural}$ obtained using the iteration scheme~\eqref{eq:PNSGD} to converge to some deterministic curve on the space of kernels $\Wcal$ in the cut norm $\cutnorm{}$ appropriately. This cannot be strengthened to the invariant $L_2$ norm $\enorm{}$. To see this, consider the sequence of processes, $\round{M_n}_{n\in\Natural}$, of $n\times n$ i.i.d. Brownian motions up to matrix symmetry. In this case, $\round{M_n}_{n\in\Natural}\to 0$ in cut norm $\cutnorm{}$ uniformly over $t\in\R_+$. But note that $\round{M_n}_{n\in\Natural}$ can not have a deterministic limit in the $L^2$ norm $\enorm{}$ for any $t>0$ due to its positive variance.

%\subsection{Interpreting non-trivial noise in SGD}\label{sec:interpreting_SGD}
% \RaghavS{More practically, what is instead used is batched SGD. To have a non-trivial continuous time interpretation of this iteration scheme, people have argued a scaling between step size and batch-size that allows them to consider this scheme as an EM discretization of a certain SDE~\cite{krizhevsky2014one,goyal2017accurate,malladi2022sdes}. We might want to add a remark about this that motivates and justifies our study on the added noise model.}

% A way to interpret ``in practice'' the noisy Stochastic Gradient Descent iteration scheme~\eqref{eq:PNSGD} is by considering a finite batch of stochastic gradients and use their average as a proxy for the true gradient for each update (see item~\ref{item:small_noise} in Section~\ref{sec:intro}). Particularly, when the batch size is scaled linearly with the step size, we recover an Euler-Maruyama iteration scheme.
% For $n\in\Natural$ and $k\in\Integer_+$, let $B_{n,k}\in\Natural$ denote the batch size of the stochastic gradients used for the $k$-th update. To take this algorithmic variation into account, let us consider $\round{\xi_{k+1,l}}_{k\in\Integer_+,l\in \Natural}$ as the i.i.d. sequence of random variables with the distribution $\Dcal$. The \emph{Projected Batched Stochastic Gradient Descent} iteration scheme starting at $W_{n,0}\in\Mcal_n$ then takes the form:
% \begin{align}
%     W_{n,k+1} = P_n\round{W_{n,k} - n^2\tau_{n,k}\cdot\inv{B_{n,k}}\sum_{l=1}^{B_{n,k}}\nabla \ell_n\round{W_{n,k};\xi_{k+1,l}}}.\label{eq:batchSGD}
% \end{align}
% Therefore, if we assume that the stochastic noise Gaussian and has a diagonal state dependent covariance, i.e., for all $n\in\Natural$, and all $A_n\in\Mcal_n$, we have
% % \[
% %     \Exp{\xi\sim\Dcal}{\abs{n^2\pdiff_{i,j} \ell_n(A_n;\xi) - n^2\pdiff_{i,j} R_n(A_n) }^2} = \Sigma_n(A_n)(i,j)^2,
% % \]
% \[
%     n^2\pdiff_{i,j} \ell_n(A_n;\xi) - n^2\pdiff_{i,j} R_n(A_n)  \sim N(0,\Sigma_n(A_n)(i,j)^2),
% \]
% for some $\Sigma_n\colon\Mcal_n \to \R_+^{\squarebrack{n}^{(2)}}$, and if the batch size $B_{n,k}$ scales linearly with the step size $\tau_{n,k}$, for example as $\tau_{n,k} = B_{n,k}$ for all $n\in\Natural$ and $k\in\Integer_+$, then~\eqref{eq:batchSGD} can be rewritten as
% \begin{align}
%     W_{n,k+1} &= P_n\round{W_{n,k} - n^2\tau_{n,k}\nabla R_n(W_{n,k}) + \tau_{n,k}^{1/2}G_{n,k}},
% \end{align}
% where $G_{n,k} \coloneqq B_{n,k}^{-1/2}\sum_{l=1}^{B_{n,k}} \round{n^2\nabla R_n(W_{n,k}) - n^2\nabla \ell_n(W_{n,k};\xi_{k+1,l})}$.

%\subsection{Stochastic Gradient Descent as an Euler Maruyama discretization of an SDE}
%SGD can also be considered as an Euler-Maruyama discretization of an SDE. For $n\in\Natural$, consider a constant step size $\tau_n > 0$. Let $B_n$ be a symmetric matrix valued process with coordinates i.i.d. Brownian motions up to matrix symmetry. Consider the SDE
%\begin{align}
%    \diff X_n(t) = -n^2 \nabla R_n(X_n(t))\diff t + \tau_n^{1/2}\sigma_n(X_n(t))\diff B_n(t),\label{eq:SME} \qquad t\in\R_+,
%\end{align}
%with initial condition $X_n(0) = W_{n,0}$ that is an $n\times n$ symmetric matrix, and $\sigma_n\colon \Mcal_n \to L(\Rd{[n]^2},\Rd{[n]^2})$.
%to the set of linear transformations from the set of $n\times n$ real symmetric matrices to itself.
%Now consider the Euler Maruyama discretization $\round{W_{n,k}}_{k\in\Integer_+}$ of the above SDE with step size $\tau_n$, i.e., given $W_{n,k}$ for any $k\in\Integer_+$,
%\[
%    W_{n,k+1} = W_{n,k} - n^2 \tau_n \nabla R_n(W_{n,k}) - \tau_n\Delta M_{n,k},
%\]
%where $\round{\Delta M_{n,k}}_{k\in\Integer_+}$ is an $n\times n$ real symmetric matrix valued martingale difference sequence, defined as
%\[
%    \Delta M_{n,k} \coloneqq \tau_n^{-1/2}\sigma_n(W_{n,k})\round{B_n((k+1)\tau_n) - B_n(k\tau_n)},\qquad k\in\Integer_+.
%\]
%If the law of $\Delta M_{n,k}$, for every $k\in\Integer_+$, coincides with the law of $n^2\nabla \ell_n(W_{n,k};\xi_{k+1}) - n^2\nabla R_n(W_{n,k})$, then we recover the SGD iteration scheme without projection (see equation~\eqref{eq:NSGD}), in law. Authors in~\cite{li2019stochastic}, develop a weak approximation framework around SDE~\eqref{eq:SME} to analyze the dynamics of SGD with positive step sizes.



\iffalse
\subsection{Analogy with mean field dynamics}
Trying to see an analogy with the mean field dynamics.
\SP{A shortened version of this discussion should go somewhere for the benefit of the reader.}

Following~\cite{song2018mean}, for any $n\in\Natural$, consider a permutation invariant function $R_n\colon \theta \mapsto R_n(\theta)\in\R$ with domain $\Rd{n}$. We can therefore consider its lifting, $R\colon\Pcal(\R)\to \R$ that satisfies $R\round{\inv{n}\sum_{i\in\squarebrack{n}}\delta_{\theta_i}} = R_n(\theta)$ for all $\theta\in\Rd{n}$ and all $n\in\Natural$. For simplicity, let us consider the noisy GD iteration scheme, but without projection. For any $n\in\Natural$, starting at $\round{\theta_{i,0}}_{i\in\squarebrack{n}}$, the noisy GD iterations take the form
\[
    \theta_{i,k+1} = \theta_{i,k} - n\tau_{n,k}\nabla R_n(\theta_{i,k}) + \beta\sqrt{\tau_{n,k}} G_{i,k},
\]
where $\round{G_{i,k}}_{i\in\squarebrack{n}}\overset{\rm i.i.d.}{\sim} N(0,1)$ for all $k\in\Integer_+$ and $\beta\in\R_+$. Notice that the first variation of $R$ at any $\rho\in\Pcal(\R)$ is $\Psi(\slot{};\rho) \colon \theta \mapsto \frac{\delta R}{\delta \rho}(\rho)(\theta)$. This motivates the definition of the {\em nonlinear dynamics}~\cite[Equations 7.4, 7.5]{song2018mean}: starting with an initialization $\round{\bar{\theta}_i(0) = \theta_i(0)}_{i\in\squarebrack{n}}$, for $t\in\R_+$,
\begin{align}
    \diff \bar{\theta}_i(t) &= -\nabla \Psi(\bar{\theta}_i(t);\rho(t))\diff t + \beta \diff B_i(t),\qquad i\in\squarebrack{n}, \qquad \rho^{(n)}(t) = \mathrm{Law}(\bar{\theta}_1(t)).\label{eq:infinite_SDE_mfd}
\end{align}
It can be seen that the trajectories $\setinline{\round{\bar{\theta}_i(t)}_{t\in\R_+}}_{n\in\Natural}$ are i.i.d. Further, it is shown in~\cite{song2018mean} that under reasonable assumptions on $R$, $(\rho(t))_{t\in\R_+}$ solves the continuity equation $\pdiff_{t}\rho(t) = \divergence\round{\rho(t)\nabla \Psi(\slot{};\rho(t))}$ at all times $t\in\R_+$. We make an analogy between equations~\eqref{eq:infinite_SDE} and~\eqref{eq:whatisgammat}, and equation~\eqref{eq:infinite_SDE_mfd}. Notice that $\round{\bar{\theta}_i(0)}_{i\in\squarebrack{n}}$ can be seen as a one dimensional exchangeable array $\round{\bar{\theta}_i(0) = f^{(n)}_0(U,U_i)}_{i\in\squarebrack{n}}$ using de Finetti's representation theorem. This is the same way as $\round{X_{n,(i,j)}(0)}_{(i,j)\in\squarebrack{n}^{(2)}}$ can be seen as a two dimensional exchangeable array $\round{X_{n,(i,j)}(0) = f^{(n)}_0(U,U_i,U_j,U_{i,j})}_{(i,j)\in\Natural^{(2)}}$ using Aldous-Hoover's representation theorem. The initial probability measure $\rho^{(n)}(0)$ can be obtained as the empirical distribution of the initialization $\round{\bar{\theta}_i(0)}_{i\in\squarebrack{n}}$ seen as a one dimensional exchangeable array for a fixed $U=u$, i.e., $\rho(0) = f^{(n)}_0(U=u,\slot{})_\sharp \lambda_{\interval{0,1}}$. The initial kernel $W_0^{(n)}$ similarly can be obtained from the initialization $\round{X_{n,(i,j)}(0)}_{(i,j)\in\squarebrack{n}^{(2)}}$ as $W_0^{(n)}(x,y) = \E{X_{n,(1,2)}(0)\given U=u,U_1=x,U_2=y}$. For $t>0$ and in the limit $n\to\infty$, we have $\rho(t) \coloneqq \lim_{n\to\infty}\rho^{(n)}(t) = \mathrm{Law}(\bar{\theta}_1(t))$, analogous to $\Gamma(t)(x,y) = \E{ X_{1,2}(t) \given U_1=x, U_2=y}$. Since $\theta(t)$ is again an exchangeable array, from de Finetti's representation theorem, there exists a function $f_t$ such that $\rho(t) = f_t(U=u,\slot{})_\sharp \lambda_{\interval{0,1}}$ for $t>0$. This implies that $\bar{\theta}_i(t)$ and $f_t(U=u,U_i)$ have the same distribution for all $i\in\Natural$. Equation~\eqref{eq:infinite_SDE_mfd} therefore reduces to
\begin{align}
    \diff \bar{\theta}_i(t) &= -\nabla \Psi\round{f_t(U=u,U_i);f_t(U=u,\slot{})_\sharp \lambda_{\interval{0,1}}}\diff t + \beta \diff B_i(t),\qquad i\in\Natural.\label{eq:infinite_SDE_mfd_withlabel_infinity}
\end{align}
Thus we can see that equation~\eqref{eq:infinite_SDE_mfd_withlabel_infinity} takes the similar form as equation~\eqref{eq:infinite_SDE}, where the role of $\Gamma$ if played by $\round{f_t}_{t\in\R_+}$, which allows us to carry the vertex labels $\round{U_i}_{i\in\Natural}$.
\fi

% \subsection{Introducing a state dependent noise (Rough thoughts)}

% Consider the PNSGD iterations of the following form. For $n\in\Natural$, starting at $W_{n,0}\in\Mcal_n$, the projected SGD algorithm produces a sequence of iterates $\round{W_{n,k}}_{k\in\Integer_+}$ defined as
% \begin{align}\label{eq:PNSGD_statedependent}
%     W_{n,k+1} = P\round{W_{n,k} - n^2\tau_{n,k}\nabla \ell_n\round{W_{n,k};\xi_{k+1}} + \beta\sqrt{\tau_{n,k}}\cdot \inv{n}S_n\round{W_{n,k}}G_{n,k}},\tag{PNSGD}
% \end{align}
% for $k\in\Integer_+$, where $S_n\colon\Mcal_n \to \Rd{\squarebrack{n}^{(2)}\times \squarebrack{n}^{(2)}}$ is the diffusion coefficient function. For $A_n\in\Mcal_n$ and $G_n\in\Rd{\squarebrack{n}^{(2)}}$, the product $S_n(A_n)G_n$ evaluates through a matrix multiplication, i.e.,
% \[
%     \round{S_n(A_n)G_n}_{(i,j)} \coloneqq \sum_{(p,q)\in\squarebrack{n}^{(2)}}S_n(A_n)_{(i,j),(p,q)}G_{n,(p,q)}, \qquad (i,j)\in\squarebrack{n}^{(2)}.
% \]
% The variance of the term $\beta\sqrt{\tau_{n,k}}\cdot \inv{n}S_n\round{W_{n,k}}G_{n,k}$ therefore is
% \begin{align*}
%     \beta^2\tau_{n,k}\cdot \frac{1}{n^2}\sum_{(p,q)\in\squarebrack{n}^{(2)}}S_n(W_{n,k})^2_{(i,j),(p,q)} &= \beta^2 \tau_{n,k} \enorm{ K\round{ S_n(W_{n,k})_{(i,j),*} } }^2. 
% \end{align*}
% This leads us to think of a modified version of~\eqref{eq:RSDE}, i.e., for $X_{n}(0)\in\Mcal_n$,
% \begin{align}
%     \begin{split}
%         \diff X_{n,(i,j)}(t) &= -n^2 \pdiff_{i,j} R_n(X_n(t))\diff t + \frac{\beta}{n}\sum_{(p,q)\in\squarebrack{n}^{(2)}}S_n(X_n(t))_{(i,j),(p,q)}\diff B_{(p,q)}(t)\\
%         &\qquad \qquad + \diff L_{n,(i,j)}^-(t) - \diff L_{n,(i,j)}^+(t), \qquad t\in\R_+, \quad (i,j)\in\squarebrack{n}^{(2)}.
%     \end{split}\label{eq:RSDE_statedependent}
% \end{align}
% A guess for generalizing equations~\eqref{eq:infinite_SDE} could be
% \begin{align}\label{eq:infinite_SDE_statedependent}
%     \diff X_{i,j}(t) &= -\phi\left( \Gamma (t)\right)(U_i, U_j)\diff t + \beta\psi\round{\Gamma(t)}(U_i,U_j,U_{i,j})\diff B_{i,j}(t) + \diff L^-_{i,j}(t) - \diff L^+_{i,j}(t),
% \end{align}
% for $t\in\R_+$, $(i,j)\in\Natural^{(2)}$, and some non-negative function $\psi\colon \Wcal \to L^2(\interval{0,1}^{(2)}\times \interval{0,1})$. The Brownian motion term used in~\eqref{eq:infinite_SDE_statedependent} is different from the one used in the finite dimensional SDE~\eqref{eq:RSDE_statedependent}, where the former is obtained from the latter through linear combinations. The solution of~\eqref{eq:infinite_SDE_statedependent} if exists, stays to be an exchangeable array. The choice for the form of the diffusion coefficient function $\psi$ is motivated through the following kind of limit:
% \[
%     \enorm{ K\round{ S_n(W_{n,k})_{(i,j),*} } } \xrightarrow[n\to\infty]{\rm Law} \psi\round{\Gamma(t)}(U_i,U_j,U_{i,j}), \qquad (i,j)\in\Natural^{(2)}, \quad t\in\R_+.
% \]
% There could be an additional term in the drift in~\eqref{eq:infinite_SDE_statedependent} due to the non-zero correlation terms in the diffusion terms for $X_{n,(i,j)}$ and $X_{n,(k,l)}$ for $(i,j)\neq (k,l)$.


%\subsection{Partially exchangeable arrays}

%Similar to symmetric exchangeable arrays, there is also a notion of partial exchangeability~\cite[Section 14]{AldExchange},~\cite{aldous1981representations}. A two dimensional array $X = \round{X_{i,j}}_{i,j\in\Natural}$ is partially exchangeable if for all finite permutations $\pi_1,\pi_2\colon\Natural\to\Natural$,
%\[
 %   \mathrm{Law}\round{\round{X_{i,j}}_{i,j\in\Natural} } = \mathrm{Law}\round{\round{X_{\pi_1(i),\pi_2(j)}}_{i,j\in\Natural}}.
%\]
%If the rows $\round{ \round{X_{i,j}}_{j\in\Natural} }_{i\in\Natural}$ and the columns $\round{ \round{X_{i,j}}_{i\in\Natural} }_{j\in\Natural}$ of $X$ are exchangeable, then $X$ is called a row column exchangeable (RCE) array. Let $\alpha$, $\set{\xi_i}_{i\in\Natural}$, $\set{\eta_j}_{j\in\Natural}$ and $\set{\lambda_{i,j}}_{i,j\in\Natural}$ be i.i.d. $\mathrm{Uni}[0,1]$ random variable. From~\cite[Theorem 14.11]{AldExchange} we have that for every RCE array $X$, there exists $f\colon\interval{0,1}^4\to\R$ such that
%\[
%    X_{i,j} \overset{\rm d}{=} f(\alpha,\xi_i,\eta_j,\lambda_{i,j}), \qquad \forall\ i,j\in\Natural.
%\]
%\RaghavS{It seems that modeling NNs using partial exchangeability makes better sense. It remains to check if the general theory of graphons also admits such a generalization.}
%\SP{The graphons are the same as the digonal block graphons. You can see that Lemma \ref{lem:random_graphon} continues to hold with a slight change.}
